Does a Global Perspective Help Prune Sparse MoEs Elegantly?

Empirical scaling laws for language models have encouraged the development of ever-larger LLMs, despite their growing computational and memory costs. Sparse Mixture-of-Experts (MoEs) offer a promising alternative by activating only a subset of experts per forward pass, improving efficiency without sacrificing performance. However, the large number of expert parameters still leads to substantial memory consumption. Existing pruning methods typically allocate budgets uniformly across layers, overlooking the heterogeneous redundancy that arises in sparse MoEs. We propose GRAPE (Global Redundancy-Aware Pruning of Experts, a global pruning strategy that dynamically allocates pruning budgets based on cross-layer redundancy. Experiments on Mixtral-8x7B, Mixtral-8x22B, DeepSeek-MoE, Qwen-MoE, and GPT-OSS show that, under the same pruning budget, GRAPE consistently achieves the best average performance. On the three main models reported in the paper, it improves average accuracy over the strongest local baseline by 1.40% on average across pruning settings, with gains of up to 2.45%.

==> tab_result.tex <==
\begin{table*}[htbp]
\centering
\caption{Results on pruning Mixtral-8x7B, Mixtral-8x22B, and DeepSeek--MoE with 2 and 4 experts per MoE layer. Each cell reports accuracy in the format $2e/4e$, where we denote $e$ as the number of experts to prune in each layer.}
\label{tab:merged_result_with_scope}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|cccccccc}
\toprule
\textbf{Model} & \textbf{Scope} & \textbf{Method} & \multicolumn{4}{c}{\textbf{MMLU}} & \textbf{BoolQ} & \textbf{OpenBookQA} & \textbf{RTE} & \textbf{Average} \\
\cmidrule(lr){4-7}
& & & Humanities & Social Science & STEM & Other & & & & \\
\midrule
\multirow{6}{*}{\textbf{Mixtral-8x7B}} 
& - & \gray{Original~\citep{jiang2024mixtral}} & \gray{60.5} & \gray{77.8} & \gray{58.9} & \gray{74.2} & \gray{85.4} & \gray{34.4} & \gray{71.1} & \gray{66.0} \\
\cmidrule(lr){2-11}
& \multirow{4}{*}{Local}
& Router-guided~\citep{li24merge} & 51.8/24.8 & 60.5/26.5 & 46.9/24.7 & 60.5/25.0 & 82.6/39.9 & 32.0/11.6 & \textbf{70.4}/50.9 & 57.8/29.1 \\
& & Count-guided~\citep{he2024demystifying} & 49.2/36.9 & 59.7/45.6 & 45.0/35.1 & 58.2/43.4 & 77.2/76.6 & 33.0/26.4 & 56.6/55.9 & 54.1/45.7 \\
& & Enumerate~\citep{lu2024not} & 52.4/43.5 & 66.4/52.7 & 49.0/40.4 & 63.7/43.5 & 84.0/80.8 & 32.6/28.8 & 71.1/66.4 & 59.9/50.8 \\
& & DEK~\citep{zhang2024diversifying} & \textbf{56.0}/48.0 & \textbf{73.1}/57.0 & 52.4/43.3 & 68.2/54.6 & \textbf{86.4}/83.3 & {31.4}/28.5 & 69.3/{67.1} & \textbf{62.4}/54.5 \\
\cmidrule(lr){2-11}
& \multirow{1}{*}{Global} & \textbf{Greedy (Ours)} & \textbf{56.0}/\textbf{48.7} & 71.0/\textbf{60.1} & \textbf{53.2}/\textbf{44.1} & \textbf{68.3}/\textbf{55.9}  & 85.1/\textbf{84.9} & \textbf{32.2}/28.4 & 69.3/66.8  & 62.2/\textbf{55.6} \\
\midrule
\multirow{6}{*}{\textbf{Mixtral-8x22B}} 
& - & \gray{Original~\citep{jiang2024mixtral}} & \gray{68.6} & \gray{84.1} & \gray{67.1} & \gray{78.7} & \gray{87.9} & \gray{35.8} & \gray{71.2} & \gray{70.4} \\
\cmidrule(lr){2-11}
& \multirow{4}{*}{Local}
& Router-guided~\citep{li24merge} & 27.3/22.7 & 25.4/25.8 & 24.4/24.0 & 27.9/23.4 & 62.8/62.7 & 12.8/13.0 & 54.2/49.5 & 33.5/31.6 \\
& & Count-guided~\citep{he2024demystifying} & 58.0/45.7 & 74.9/57.7 & 54.1/42.0 & 70.2/45.7 & 81.5/74.4 & 35.2/27.0 & 69.3/57.4 & 63.3/50.0 \\
& & Enumerate~\citep{lu2024not} & 60.4/53.9 & 78.0/67.2 & 59.5/52.3 & 73.0/64.2 & 87.4/80.5 & 35.0/31.1 & 70.1/67.9 & 66.2/59.6 \\
& & DEK~\citep{zhang2024diversifying} & 62.3/57.8 & 78.5/69.7 & 60.2/51.3 & 73.4/64.2 & 87.6/83.1 & \textbf{35.8}/33.2 & \textbf{71.1}/68.1 & 67.0/61.1 \\
\cmidrule(lr){2-11}
& \multirow{1}{*}{Global} & \textbf{Greedy (Ours)} & \textbf{64.1}/\textbf{58.4} & \textbf{80.4}/\textbf{72.9} & \textbf{62.7}/\textbf{54.6} & \textbf{75.3}/\textbf{67.9} & \textbf{88.0}/\textbf{84.1}  & 35.2/32.0 & \textbf{71.4}/\textbf{68.5}  & \textbf{68.2}/\textbf{62.6}  \\
\midrule
\multirow{5}{*}{\textbf{Deepseek-MoE}} 
& - & \gray{Original~\citep{dai2024deepseekmoe}} & 40.4 & 47.9 & 36.1 & 49.5  & 77.2 & 32.8 & 66.0 & 50.0 \\
\cmidrule(lr){2-11}
& \multirow{3}{*}{Local}
& Router-guided~\citep{li24merge} & 38.1/34.3 & 46.4/41.6 & 33.9/33.6 & 47.7/43.1 & 71.3/72.1  & 33.2/31.4 & 60.4/60.2 & 47.3/45.2 \\
& & Count-guided~\citep{he2024demystifying} & 38.3/35.9 & 47.4/42.5 & 34.1/32.9 & 47.4/45.6 & 76.2/75.9 & \textbf{33.8}/\textbf{32.4} & 64.9/\textbf{67.5} & 48.9/47.5  \\
& & DEK~\citep{zhang2024diversifying} & 38.7/{39.2} & 47.3/{47.0} & {34.9}/{33.7} & 46.9/{46.6} & 77.4/{76.6} & 32.2/32.2 &64.6/66.4  & 48.8/{48.8} \\
\cmidrule(lr){2-11}
& {Global} & \textbf{Greedy (Ours)} & \textbf{39.7}/\textbf{39.7} & \textbf{48.3}/\textbf{47.6} & \textbf{35.8}/\textbf{35.3} & \textbf{50.0}/\textbf{50.0}  & \textbf{77.8}/\textbf{77.5}  & {32.0}/31.2 &  \textbf{65.0}/65.5 &  \textbf{49.8}/\textbf{49.5} \\
\midrule
\multirow{6}{*}{\textbf{Qwen-MoE}} 
& - & \gray{Original~\citep{dai2024deepseekmoe}} & 53.6 & 70.0 & 51.2 & 67.4 & 81.3 & 33.2 & 77.2 & 62.0 \\
\cmidrule(lr){2-11}
& \multirow{3}{*}{Local}
& Router-guided~\citep{li24merge} & 51.2/50.0  & {69.7}/66.5 & 50.7/49.3 & {67.4}/64.8 &  76.6/78.2 & \textbf{33.8}/\textbf{33.4}  & 76.1/74.7 & 60.7/59.5 \\
& & Count-guided~\citep{he2024demystifying} & 52.1/50.6  & 69.0/67.2  & \textbf{51.3}/{50.3} & 66.9/{66.1}  & 79.2/\textbf{81.3}  & 33.4/\textbf{33.4} & 71.8/74.0 & 60.5/60.4 \\
& & DEK~\citep{zhang2024diversifying} & {52.8}/{52.5} & 69.1/{68.7} & 50.9/50.0 & 66.7/65.9 & \textbf{81.2}/\textbf{81.3}  &  33.2/33.2 & \textbf{77.6}/\textbf{76.9} & {61.7}/{61.2} \\
\cmidrule(lr){2-11} 
& {Global} & \textbf{Greedy (Ours)} &  \textbf{54.1}/\textbf{53.7} & \textbf{69.8}/\textbf{69.1}  & \textbf{51.3}/\textbf{51.3}  &  \textbf{67.2}/\textbf{66.7} & \textbf{81.2}/81.0  & 33.4/31.4 & 75.7/76.5 &  \textbf{61.8}/\textbf{61.4} \\
\midrule
\multirow{5}{*}{\textbf{GPT-oss}} 
& - & \gray{Original~\citep{dai2024deepseekmoe}} & 44.9  & 65.3  & 50.0  & 70.8 & 75.8 & 27.0 & 68.2 & 57.3\\
\cmidrule(lr){2-11}
& \multirow{3}{*}{Local}
& Router-guided~\citep{li24merge} & 42.8/41.9  & 64.9/63.5  & 49.1/47.3  & 70.4/69.2  & 74.8/74.2  & 26.2/26.4 & 71.2/71.5  & 57.1/56.3  \\
& & Count-guided~\citep{he2024demystifying} & 43.5/43.8  & 65.5/64.9  & 47.9/47.1  & 70.6/70.8 & 75.4/74.7  & 26.6/26.0 & 69.7/68.2 &  57.0/56.0\\
& & DEK~\citep{zhang2024diversifying}  

& 43.9/39.6
& 62.2/55.2
& 46.7/41.9
& 66.0/62.4
& 74.8/71.3
& 25.8/24.0
& 66.4/65.0
& 55.1/51.3    \\

\cmidrule(lr){2-11}
& {Global} & \textbf{Greedy (Ours)} & 45.2/44.7  & 66.3/65.3 & 49.5/48.2  &  71.4/71.4  & 76.0/75.3  & 26.9/26.3  & 68.4/67.5 & 57.7/57.0 \\ 
\bottomrule
\end{tabular}}
\end{table*}


